Encyclo-K: Evaluating LLMs with Dynamically Composed Knowledge Statements

Benchmarks play a crucial role in tracking the rapid advancement of large language models (LLMs) and identifying their capability boundaries. However, existing benchmarks predominantly curate questions at the question level, suffering from three fundamental limitations: vulnerability to data contamination, restriction to single-knowledge-point assessment, and reliance on costly domain expert annotation. We propose Encyclo-K, a statement-based benchmark that rethinks benchmark construction from the ground up. Our key insight is that knowledge statements, not questions, can serve as the unit of curation, and questions can then be constructed from them. We extract standalone knowledge statements from authoritative textbooks and dynamically compose them into evaluation questions through random sampling at test time. This design directly addresses all three limitations: the combinatorial space is too vast to memorize, and model rankings remain stable across dynamically generated question sets, enabling reliable periodic dataset refresh; each question aggregates 8-10 statements for comprehensive multi-knowledge assessment; annotators only verify formatting compliance without requiring domain expertise, substantially reducing annotation costs. Experiments on over 50 LLMs demonstrate that Encyclo-K poses substantial challenges with strong discriminative power. Even the top-performing OpenAI-GPT-5.1 achieves only 62.07% accuracy, and model performance displays a clear gradient distribution--reasoning models span from 16.04% to 62.07%, while chat models range from 9.71% to 50.40%. These results validate the challenges introduced by dynamic evaluation and multi-statement comprehensive understanding. These findings establish Encyclo-K as a scalable framework for dynamic evaluation of LLMs' comprehensive understanding over multiple fine-grained disciplinary knowledge statements.

==> sections/results/performance_1.tex <==
\definecolor{color11}{rgb}{1, 0.8, 0.8}  % 红色20%混合
\definecolor{color12}{rgb}{1, 0.9, 0.9}  % 红色10%混合
\definecolor{color21}{RGB}{255, 224, 127}  % 更亮的黄色调，温暖
\definecolor{color22}{RGB}{255, 239, 179}  % 浅黄色调，亮度增加
\definecolor{color31}{RGB}{198, 230, 195}  % 更亮的绿色，柔和清新
\definecolor{color32}{RGB}{224, 239, 225}  % 更亮的浅绿色，清新且明亮

{
\linespread{1}
\begin{table}[H]
\scriptsize
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{4cm}<{\raggedright\arraybackslash}*{7}{p{2cm}<{\centering\arraybackslash}}}
\toprule
\textbf{Model} & \textbf{Overall} & \textbf{Overall} & \textbf{Overall} & \textbf{Overall} & \textbf{Easy} & \textbf{Middle} & \textbf{Hard}\\
& \textbf{(sample)} & \textbf{(subfield)} & \textbf{(field)} & \textbf{(discipline)} & \textbf{(sample)} & \textbf{(sample)} & \textbf{(sample)}\\
\midrule
\rowcolor{color11}
\multicolumn{8}{c}{\textbf{\textit{Reasoning Models}}}\\
\midrule
\rowcolor{color12}
DeepSeek-R1 &\boxed{61.82} & \boxed{62.61} & \boxed{61.23} & \textbf{59.95} & \underline{63.59} & \boxed{63.63} &\boxed{56.87} \\
\rowcolor{color12}
o1-2024-12-17 &\textbf{60.24} & \underline{61.25} & \underline{59.94} & \underline{59.44} & \textbf{64.40} & \underline{61.44} &\underline{53.67} \\
\rowcolor{color12}
DeepSeek-R1-Zero &\textbf{60.24} & \textbf{61.62} & \textbf{60.95} & \boxed{60.99} & \boxed{65.06} & \textbf{62.61} &50.99 \\
\rowcolor{color12}
o3-mini-2025-01-31-high &\underline{55.22} & 54.94 & 52.11 & 48.32 & 53.05 & 56.09 &\textbf{56.16} \\
\rowcolor{color12}
o3-mini-2025-01-31-medium &52.69 & 52.66 & 49.95 & 46.07 & 51.30 & 53.79 &52.37 \\
\rowcolor{color12}
o3-mini-2025-01-31-low &48.03 & 48.51 & 45.89 & 42.63 & 48.80 & 50.21 &43.53 \\
\rowcolor{color12}
o1-mini-2024-09-12 &45.22 & 45.46 & 42.53 & 39.33 & 46.77 & 47.34 &40.00 \\
\rowcolor{color12}
QwQ &43.59 & 44.40 & 43.19 & 41.63 & 46.46 & 47.40 &34.07 \\
\midrule
\rowcolor{color21}
\multicolumn{8}{c}{\textbf{\textit{Chat Models}}}\\
\midrule
\rowcolor{color22}
Doubao-1.5-pro-32k-250115 &\boxed{55.09} & \boxed{56.55} & \boxed{55.62} & \boxed{54.39} & \underline{57.70} & \boxed{60.15} &\boxed{43.80} \\
\rowcolor{color22}
Doubao-1.5-pro-32k-241225 &\textbf{50.93} & \underline{52.41} & \underline{51.76} & 51.24 & 53.54 & \textbf{56.56} &\underline{38.70} \\
\rowcolor{color22}
qwen-max-2025-01-25 &\underline{50.08} & \textbf{52.75} & \textbf{52.47} & \underline{51.65} & \textbf{58.16} & \underline{54.95} &33.09 \\
\rowcolor{color22}
claude-3-5-sonnet-20241022 &48.16 & 51.38 & 51.23 & \textbf{53.15} & \boxed{59.04} & 51.91 &29.99 \\
\rowcolor{color22}
gemini-2.0-flash &47.73 & 48.70 & 47.80 & 46.10 & 53.06 & 49.56 &\textbf{38.84} \\
\rowcolor{color22}
DeepSeek-V3 &47.40 & 49.10 & 48.31 & 47.35 & 55.63 & 50.11 &33.86 \\
\rowcolor{color22}
MiniMax-Text-01 &45.11 & 47.46 & 46.97 & 47.06 & 54.51 & 48.60 &28.98 \\
\rowcolor{color22}
gpt-4o-2024-11-20 &44.40 & 47.62 & 47.50 & 48.84 & 56.84 & 48.75 &23.50 \\
\rowcolor{color22}
Llama-3.1-405B-Instruct &43.14 & 46.43 & 45.83 & 47.35 & 56.06 & 46.31 &23.70 \\
\rowcolor{color22}
gpt-4o-2024-08-06 &41.64 & 44.79 & 44.91 & 46.29 & 55.22 & 45.11 &20.98 \\
\rowcolor{color22}
Qwen2.5-72B-Instruct &40.75 & 43.66 & 43.32 & 42.10 & 48.84 & 45.42 &24.10 \\
\rowcolor{color22}
Mistral-Large-Instruct-2411 &40.65 & 43.38 & 43.13 & 43.37 & 52.92 & 43.28 &22.81 \\
\rowcolor{color22}
qwen-max-2024-09-19 &39.96 & 42.93 & 42.16 & 41.62 & 50.23 & 43.63 &22.60 \\
\rowcolor{color22}
gpt-4o-2024-05-13 &39.76 & 43.19 & 43.13 & 45.23 & 53.37 & 42.38 &20.45 \\
\rowcolor{color22}
Qwen2.5-32B-Instruct &38.76 & 41.18 & 40.40 & 39.43 & 47.42 & 43.05 &22.13 \\
\rowcolor{color22}
Llama-3.3-70B-Instruct &37.69 & 40.56 & 40.15 & 41.12 & 49.68 & 40.68 &19.55 \\
\rowcolor{color22}
phi-4 &37.65 & 39.59 & 38.61 & 37.66 & 45.43 & 40.91 &23.69 \\
\rowcolor{color22}
Qwen2.5-14B-Instruct &35.15 & 37.72 & 37.41 & 36.07 & 44.82 & 37.90 &19.97 \\
\rowcolor{color22}
Llama-3.1-70B-Instruct &34.86 & 38.94 & 39.18 & 40.57 & 48.22 & 37.85 &15.22 \\
\rowcolor{color22}
Yi-Lightning &33.42 & 36.57 & 36.45 & 36.92 & 43.38 & 35.32 &19.35 \\
\rowcolor{color22}
Mixtral-8x22B-Instruct-v0.1 &29.23 & 32.14 & 32.28 & 32.82 & 42.52 & 29.73 &13.82 \\
\rowcolor{color22}
Qwen2.5-7B-Instruct &28.78 & 30.78 & 30.37 & 30.63 & 37.77 & 30.98 &15.23 \\
\rowcolor{color22}
gemma-2-27b-it &27.43 & 30.50 & 30.42 & 31.30 & 40.90 & 27.45 &12.64 \\
\rowcolor{color22}
Yi-1.5-34B-Chat &26.03 & 28.81 & 28.84 & 29.08 & 36.99 & 26.74 &12.81 \\
\rowcolor{color22}
Mistral-Small-Instruct-2409 &25.89 & 28.46 & 28.69 & 28.59 & 37.93 & 25.89 &12.70 \\
\rowcolor{color22}
gemma-2-9b-it &24.04 & 26.89 & 27.06 & 27.74 & 37.81 & 23.05 &10.60 \\
\rowcolor{color22}
Qwen2.5-3B-Instruct &23.31 & 25.45 & 25.86 & 25.57 & 33.10 & 23.50 &12.24 \\
\rowcolor{color22}
Yi-1.5-9B-Chat &23.17 & 25.32 & 25.65 & 26.07 & 32.75 & 24.05 &11.19 \\
\rowcolor{color22}
K2-Chat &22.47 & 24.59 & 24.61 & 24.61 & 30.58 & 21.95 &14.44 \\
\rowcolor{color22}
Mixtral-8x7B-Instruct-v0.1 &22.10 & 24.76 & 24.73 & 26.36 & 34.19 & 20.52 &11.49 \\
\rowcolor{color22}
granite-3.1-8b-instruct &20.83 & 22.85 & 22.92 & 22.26 & 29.48 & 19.79 &13.09 \\
\rowcolor{color22}
Llama-3.1-8B-Instruct &20.50 & 24.07 & 24.52 & 26.12 & 32.82 & 20.37 &7.22 \\
\rowcolor{color22}
Yi-1.5-6B-Chat &19.24 & 21.32 & 21.39 & 22.21 & 27.90 & 18.83 &10.44 \\
\rowcolor{color22}
Qwen2.5-1.5B-Instruct &18.82 & 20.91 & 20.75 & 22.11 & 27.41 & 18.19 &10.45 \\
\rowcolor{color22}
OLMo-2-1124-13B-Instruct &18.66 & 20.46 & 20.60 & 21.80 & 27.10 & 17.85 &10.74 \\
\rowcolor{color22}
gemma-2-2b-it &18.61 & 19.91 & 19.97 & 20.50 & 26.40 & 16.95 &12.85 \\
\rowcolor{color22}
granite-3.1-2b-instruct &17.92 & 19.02 & 19.11 & 19.58 & 23.94 & 17.58 &11.87 \\
\rowcolor{color22}
Mistral-7B-Instruct-v0.3 &17.82 & 19.64 & 19.65 & 20.09 & 26.37 & 16.64 &10.41 \\
\rowcolor{color22}
MAP-Neo-7B-Instruct-v0.1 &17.05 & 18.52 & 18.42 & 18.70 & 23.26 & 16.62 &10.95 \\
\rowcolor{color22}
OLMo-2-1124-7B-Instruct &16.81 & 18.08 & 18.57 & 18.85 & 22.80 & 15.82 &11.90 \\
\rowcolor{color22}
Qwen2.5-0.5B-Instruct &10.77 & 11.92 & 12.47 & 13.47 & 14.90 & 10.88 &6.07 \\
\midrule
\rowcolor{color31}
\multicolumn{8}{c}{\textbf{\textit{Base Models}}}\\
\midrule
\rowcolor{color32}
Qwen2.5-72B & \boxed{34.33} & \boxed{38.08} & \boxed{38.70} & \boxed{39.54} & \boxed{46.20} & \boxed{38.12} &\textbf{15.01} \\
\rowcolor{color32}
Qwen2.5-32B & \textbf{33.16} & \textbf{36.52} & \textbf{37.33} & \textbf{38.29} & \textbf{45.12} & \textbf{36.58} &14.34 \\
\rowcolor{color32}
DeepSeek-V3-Base & \underline{32.14} & \underline{34.79} & \underline{34.58} & \underline{34.71} & 41.28 & \underline{34.50} &\boxed{18.20} \\
\rowcolor{color32}
Qwen2.5-14B & 30.19 & 33.33 & 34.14 & 34.54 & \underline{42.27} & 31.44 &\underline{14.85} \\
\rowcolor{color32}
Yi-1.5-34B & 27.62 & 30.78 & 31.03 & 32.55 & 39.68 & 27.95 &13.86 \\
\rowcolor{color32}
Llama-3.1-70B & 27.22 & 30.52 & 31.28 & 32.55 & 40.78 & 26.95 &12.78 \\
\rowcolor{color32}
Qwen2.5-7B & 25.36 & 28.19 & 28.73 & 29.60 & 36.58 & 25.94 &12.10 \\
\rowcolor{color32}
Llama-3.1-405B & 25.23 & 28.09 & 28.33 & 30.15 & 37.58 & 25.12 &11.86 \\
\rowcolor{color32}
gemma-2-27b & 24.49 & 27.35 & 27.96 & 28.58 & 36.26 & 24.07 &12.27 \\
\rowcolor{color32}
Yi-1.5-9B & 23.10 & 25.40 & 25.69 & 26.17 & 32.52 & 22.98 &12.96 \\
\rowcolor{color32}
gemma-2-9b & 22.56 & 25.19 & 25.47 & 26.26 & 33.88 & 21.34 &12.20 \\
\rowcolor{color32}
Mixtral-8x22B-v0.1 & 22.41 & 24.71 & 25.04 & 25.02 & 32.78 & 21.67 &12.26 \\
\rowcolor{color32}
Mixtral-8x7B-v0.1 & 21.76 & 24.92 & 25.45 & 27.36 & 33.66 & 20.32 &11.13 \\
\rowcolor{color32}
K2 & 20.92 & 23.62 & 23.88 & 24.65 & 30.97 & 20.01 &11.40 \\
\rowcolor{color32}
Yi-1.5-6B & 20.20 & 22.10 & 22.56 & 23.44 & 28.37 & 19.64 &12.20 \\
\rowcolor{color32}
Qwen2.5-3B & 20.14 & 22.81 & 23.30 & 24.42 & 30.42 & 19.81 &9.40 \\
\rowcolor{color32}
Llama-3.1-8B & 19.93 & 22.42 & 22.77 & 23.87 & 30.33 & 18.94 &10.16 \\
\rowcolor{color32}
Mistral-7B-v0.3 & 19.48 & 21.50 & 21.81 & 22.27 & 27.62 & 18.65 &11.96 \\
\rowcolor{color32}
Qwen2.5-1.5B & 17.17 & 19.31 & 19.80 & 21.35 & 24.52 & 16.79 &9.74 \\
\rowcolor{color32}
granite-3.1-2b-base & 16.18 & 17.90 & 17.91 & 18.09 & 23.13 & 14.91 &10.67 \\
\rowcolor{color32}
OLMo-2-1124-13B & 16.07 & 18.75 & 19.82 & 21.37 & 27.24 & 14.41 &6.57 \\
\rowcolor{color32}
MAP-Neo-7B & 15.76 & 17.48 & 18.26 & 19.54 & 22.86 & 14.64 &9.83 \\
\rowcolor{color32}
granite-3.1-8b-base & 15.69 & 16.98 & 16.79 & 16.65 & 20.40 & 15.65 &10.60 \\
\rowcolor{color32}
OLMo-2-1124-7B & 15.15 & 17.62 & 18.30 & 19.60 & 24.43 & 13.83 &7.15 \\
\rowcolor{color32}
gemma-2-2b & 13.57 & 14.98 & 15.43 & 16.21 & 19.12 & 13.47 &7.63 \\
\rowcolor{color32}
Qwen2.5-0.5B & 10.74 & 11.88 & 12.09 & 13.25 & 14.41 & 10.78 &6.65 \\

\bottomrule
\end{tabular}
}
\captionsetup{font=footnotesize}
\caption{\textbf{Detailed Performance Overview on \benchmark - Pivot Table 1.} 
LLMs are scored sample-wise, subfield-wise, field-wise, and discipline-wise levels to ensure fair assessment despite imbalanced question counts. 
The columns Easy(sample), Middle(sample), and Hard(sample) represent average scores according to difficulty. 
The highest score in each column is indicated with a \boxed{box}; the second-best score is in \textbf{bold}, and the third-best score is \underline{underlined}.}
\label{performance1_all}
\end{table}
}


==> sections/results/performance_1_main.tex <==
\definecolor{color11}{rgb}{1, 0.8, 0.8}  % 红色20%混合
\definecolor{color12}{rgb}{1, 0.9, 0.9}  % 红色10%混合
\definecolor{color21}{RGB}{255, 224, 127}  % 更亮的黄色调，温暖
\definecolor{color22}{RGB}{255, 239, 179}  % 浅黄色调，亮度增加
\definecolor{color31}{RGB}{198, 230, 195}  % 更亮的绿色，柔和清新
\definecolor{color32}{RGB}{224, 239, 225}  % 更亮的浅绿色，清新且明亮
% \newgeometry{top=2cm,bottom=2cm} % 第一页特殊边距

{
\linespread{1.1}
\begin{table}[p]
\small
\centering
\setlength{\tabcolsep}{3pt} 
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{6.6pt}
\begin{tabular}{p{4.5cm}<{\raggedright\arraybackslash}*{7}{p{1.6cm}<{\centering\arraybackslash}}}
\toprule
\textbf{Model} & \textbf{Overall} & \textbf{Overall} & \textbf{Overall} & \textbf{Overall} & \textbf{Easy} & \textbf{Middle} & \textbf{Hard}\\
& \textbf{(sample)} & \textbf{(subfield)} & \textbf{(field)} & \textbf{(discipline)} & \textbf{(sample)} & \textbf{(sample)} & \textbf{(sample)}\\
\midrule
\rowcolor{color11}
\multicolumn{8}{c}{\textbf{\textit{Reasoning Models}}}\\
\midrule
\rowcolor{color12}
DeepSeek-R1 &\boxed{61.82} & \boxed{62.61} & \boxed{61.23} & \textbf{59.95} & \underline{63.59} & \boxed{63.63} &\boxed{56.87} \\
\rowcolor{color12}
o1-2024-12-17 &\textbf{60.24} & \underline{61.25} & \underline{59.94} & \underline{59.44} & \textbf{64.40} & \underline{61.44} &\underline{53.67} \\
\rowcolor{color12}
DeepSeek-R1-Zero &\textbf{60.24} & \textbf{61.62} & \textbf{60.95} & \boxed{60.99} & \boxed{65.06} & \textbf{62.61} &50.99 \\
\rowcolor{color12}
o3-mini-2025-01-31-high &\underline{55.22} & 54.94 & 52.11 & 48.32 & 53.05 & 56.09 &\textbf{56.16} \\
\rowcolor{color12}
o3-mini-2025-01-31-medium &52.69 & 52.66 & 49.95 & 46.07 & 51.30 & 53.79 &52.37 \\
\rowcolor{color12}
o3-mini-2025-01-31-low &48.03 & 48.51 & 45.89 & 42.63 & 48.80 & 50.21 &43.53 \\
\rowcolor{color12}
o1-mini-2024-09-12 &45.22 & 45.46 & 42.53 & 39.33 & 46.77 & 47.34 &40.00 \\
\rowcolor{color12}
QwQ &43.59 & 44.40 & 43.19 & 41.63 & 46.46 & 47.40 &34.07 \\
\midrule
\rowcolor{color21}
\multicolumn{8}{c}{\textbf{\textit{Chat Models}}}\\
\midrule
\rowcolor{color22}
Doubao-1.5-pro-32k-250115 &\boxed{55.09} & \boxed{56.55} & \boxed{55.62} & \boxed{54.39} & \underline{57.70} & \boxed{60.15} &\boxed{43.80} \\
\rowcolor{color22}
Doubao-1.5-pro-32k-241225 &\textbf{50.93} & \underline{52.41} & \underline{51.76} & 51.24 & 53.54 & \textbf{56.56} &\underline{38.70} \\
\rowcolor{color22}
Qwen-max-2025-01-25 &\underline{50.08} & \textbf{52.75} & \textbf{52.47} & \underline{51.65} & \textbf{58.16} & \underline{54.95} &33.09 \\
\rowcolor{color22}
Claude-3-5-sonnet-20241022 &48.16 & 51.38 & 51.23 & \textbf{53.15} & \boxed{59.04} & 51.91 &29.99 \\
\rowcolor{color22}
Gemini-2.0-flash &47.73 & 48.70 & 47.80 & 46.10 & 53.06 & 49.56 &\textbf{38.84} \\
\rowcolor{color22}
DeepSeek-V3 &47.40 & 49.10 & 48.31 & 47.35 & 55.63 & 50.11 &33.86 \\
\rowcolor{color22}
MiniMax-Text-01 &45.11 & 47.46 & 46.97 & 47.06 & 54.51 & 48.60 &28.98 \\
\rowcolor{color22}
GPT-4o-2024-11-20 &44.40 & 47.62 & 47.50 & 48.84 & 56.84 & 48.75 &23.50 \\
\rowcolor{color22}
Llama-3.1-405B-Instruct &43.14 & 46.43 & 45.83 & 47.35 & 56.06 & 46.31 &23.70 \\
\rowcolor{color22}
GPT-4o-2024-08-06 &41.64 & 44.79 & 44.91 & 46.29 & 55.22 & 45.11 &20.98 \\
\rowcolor{color22}
Qwen2.5-72B-Instruct &40.75 & 43.66 & 43.32 & 42.10 & 48.84 & 45.42 &24.10 \\
\rowcolor{color22}
Mistral-Large-Instruct-2411 &40.65 & 43.38 & 43.13 & 43.37 & 52.92 & 43.28 &22.81 \\
\rowcolor{color22}
Qwen-max-2024-09-19 &39.96 & 42.93 & 42.16 & 41.62 & 50.23 & 43.63 &22.60 \\
% \rowcolor{color22}
% gpt-4o-2024-05-13 &39.76 & 43.19 & 43.13 & 45.23 & 53.37 & 42.38 &20.45 \\
\rowcolor{color22}
Qwen2.5-32B-Instruct &38.76 & 41.18 & 40.40 & 39.43 & 47.42 & 43.05 &22.13 \\
\rowcolor{color22}
Llama-3.3-70B-Instruct &37.69 & 40.56 & 40.15 & 41.12 & 49.68 & 40.68 &19.55 \\
\rowcolor{color22}
Phi-4 &37.65 & 39.59 & 38.61 & 37.66 & 45.43 & 40.91 &23.69 \\
\rowcolor{color22}
Qwen2.5-14B-Instruct &35.15 & 37.72 & 37.41 & 36.07 & 44.82 & 37.90 &19.97 \\
\rowcolor{color22}
Llama-3.1-70B-Instruct &34.86 & 38.94 & 39.18 & 40.57 & 48.22 & 37.85 &15.22 \\
\rowcolor{color22}
Yi-Lightning &33.42 & 36.57 & 36.45 & 36.92 & 43.38 & 35.32 &19.35 \\
\rowcolor{color22}
Mixtral-8x22B-Instruct-v0.1 &29.23 & 32.14 & 32.28 & 32.82 & 42.52 & 29.73 &13.82 \\
\rowcolor{color22}
Qwen2.5-7B-Instruct &28.78 & 30.78 & 30.37 & 30.63 & 37.77 & 30.98 &15.23 \\
\rowcolor{color22}
Gemma-2-27B-it &27.43 & 30.50 & 30.42 & 31.30 & 40.90 & 27.45 &12.64 \\
% \rowcolor{color22}
% Yi-1.5-34B-Chat &26.03 & 28.81 & 28.84 & 29.08 & 36.99 & 26.74 &12.81 \\
% \rowcolor{color22}
% Mistral-Small-Instruct-2409 &25.89 & 28.46 & 28.69 & 28.59 & 37.93 & 25.89 &12.70 \\
% \rowcolor{color22}
% gemma-2-9b-it &24.04 & 26.89 & 27.06 & 27.74 & 37.81 & 23.05 &10.60 \\
\rowcolor{color22}
Qwen2.5-3B-Instruct &23.31 & 25.45 & 25.86 & 25.57 & 33.10 & 23.50 &12.24 \\
% \rowcolor{color22}
% Yi-1.5-9B-Chat &23.17 & 25.32 & 25.65 & 26.07 & 32.75 & 24.05 &11.19 \\
% \rowcolor{color22}
% K2-Chat &22.47 & 24.59 & 24.61 & 24.61 & 30.58 & 21.95 &14.44 \\
% \rowcolor{color22}
% Mixtral-8x7B-Instruct-v0.1 &22.10 & 24.76 & 24.73 & 26.36 & 34.19 & 20.52 &11.49 \\
\rowcolor{color22}
Granite-3.1-8B-instruct &20.83 & 22.85 & 22.92 & 22.26 & 29.48 & 19.79 &13.09 \\
% \rowcolor{color22}
% Llama-3.1-8B-Instruct &20.50 & 24.07 & 24.52 & 26.12 & 32.82 & 20.37 &7.22 \\
% \rowcolor{color22}
% Yi-1.5-6B-Chat &19.24 & 21.32 & 21.39 & 22.21 & 27.90 & 18.83 &10.44 \\
\rowcolor{color22}
Qwen2.5-1.5B-Instruct &18.82 & 20.91 & 20.75 & 22.11 & 27.41 & 18.19 &10.45 \\
\rowcolor{color22}
OLMo-2-1124-13B-Instruct &18.66 & 20.46 & 20.60 & 21.80 & 27.10 & 17.85 &10.74 \\
% \rowcolor{color22}
% gemma-2-2b-it &18.61 & 19.91 & 19.97 & 20.50 & 26.40 & 16.95 &12.85 \\
% \rowcolor{color22}
% granite-3.1-2b-instruct &17.92 & 19.02 & 19.11 & 19.58 & 23.94 & 17.58 &11.87 \\
% \rowcolor{color22}
% Mistral-7B-Instruct-v0.3 &17.82 & 19.64 & 19.65 & 20.09 & 26.37 & 16.64 &10.41 \\
\rowcolor{color22}
MAP-Neo-7B-Instruct-v0.1 &17.05 & 18.52 & 18.42 & 18.70 & 23.26 & 16.62 &10.95 \\
\rowcolor{color22}
OLMo-2-1124-7B-Instruct &16.81 & 18.08 & 18.57 & 18.85 & 22.80 & 15.82 &11.90 \\
% \rowcolor{color22}
% Qwen2.5-0.5B-Instruct &10.77 & 11.92 & 12.47 & 13.47 & 14.90 & 10.88 &6.07 \\
\midrule
\rowcolor{color31}
\multicolumn{8}{c}{\textbf{\textit{Base Models}}}\\
\midrule
\rowcolor{color32}
Qwen2.5-72B & \boxed{34.33} & \boxed{38.08} & \boxed{38.70} & \boxed{39.54} & \boxed{46.20} & \boxed{38.12} &\textbf{15.01} \\
\rowcolor{color32}
Qwen2.5-32B & \textbf{33.16} & \textbf{36.52} & \textbf{37.33} & \textbf{38.29} & \textbf{45.12} & \textbf{36.58} &14.34 \\
\rowcolor{color32}
DeepSeek-V3-Base & \underline{32.14} & \underline{34.79} & \underline{34.58} & \underline{34.71} & 41.28 & \underline{34.50} &\boxed{18.20} \\
\rowcolor{color32}
Qwen2.5-14B & 30.19 & 33.33 & 34.14 & 34.54 & \underline{42.27} & 31.44 &\underline{14.85} \\
\rowcolor{color32}
Yi-1.5-34B & 27.62 & 30.78 & 31.03 & 32.55 & 39.68 & 27.95 &13.86 \\
\rowcolor{color32}
Llama-3.1-70B & 27.22 & 30.52 & 31.28 & 32.55 & 40.78 & 26.95 &12.78 \\
\rowcolor{color32}
Qwen2.5-7B & 25.36 & 28.19 & 28.73 & 29.60 & 36.58 & 25.94 &12.10 \\
\rowcolor{color32}
Llama-3.1-405B & 25.23 & 28.09 & 28.33 & 30.15 & 37.58 & 25.12 &11.86 \\
\rowcolor{color32}
Gemma-2-27B & 24.49 & 27.35 & 27.96 & 28.58 & 36.26 & 24.07 &12.27 \\
\rowcolor{color32}
% Yi-1.5-9B & 23.10 & 25.40 & 25.69 & 26.17 & 32.52 & 22.98 &12.96 \\
% \rowcolor{color32}
% gemma-2-9b & 22.56 & 25.19 & 25.47 & 26.26 & 33.88 & 21.34 &12.20 \\
% \rowcolor{color32}
Mixtral-8x22B-v0.1 & 22.41 & 24.71 & 25.04 & 25.02 & 32.78 & 21.67 &12.26 \\
\rowcolor{color32}
% Mixtral-8x7B-v0.1 & 21.76 & 24.92 & 25.45 & 27.36 & 33.66 & 20.32 &11.13 \\
% \rowcolor{color32}
% K2 & 20.92 & 23.62 & 23.88 & 24.65 & 30.97 & 20.01 &11.40 \\
% \rowcolor{color32}
% Yi-1.5-6B & 20.20 & 22.10 & 22.56 & 23.44 & 28.37 & 19.64 &12.20 \\
\rowcolor{color32}
Qwen2.5-3B & 20.14 & 22.81 & 23.30 & 24.42 & 30.42 & 19.81 &9.40 \\
% \rowcolor{color32}
% Llama-3.1-8B & 19.93 & 22.42 & 22.77 & 23.87 & 30.33 & 18.94 &10.16 \\
\rowcolor{color32}
Mistral-7B-v0.3 & 19.48 & 21.50 & 21.81 & 22.27 & 27.62 & 18.65 &11.96 \\
\rowcolor{color32}
Qwen2.5-1.5B & 17.17 & 19.31 & 19.80 & 21.35 & 24.52 & 16.79 &9.74 \\
% \rowcolor{color32}
% granite-3.1-2b-base & 16.18 & 17.90 & 17.91 & 18.09 & 23.13 & 14.91 &10.67 \\
\rowcolor{color32}
OLMo-2-1124-13B & 16.07 & 18.75 & 19.82 & 21.37 & 27.24 & 14.41 &6.57 \\
\rowcolor{color32}
MAP-Neo-7B & 15.76 & 17.48 & 18.26 & 19.54 & 22.86 & 14.64 &9.83 \\
\rowcolor{color32}
Granite-3.1-8B-Base & 15.69 & 16.98 & 16.79 & 16.65 & 20.40 & 15.65 &10.60 \\
\rowcolor{color32}
OLMo-2-1124-7B & 15.15 & 17.62 & 18.30 & 19.60 & 24.43 & 13.83 &7.15 \\
% \rowcolor{color32}
% gemma-2-2b & 13.57 & 14.98 & 15.43 & 16.21 & 19.12 & 13.47 &7.63 \\
% \rowcolor{color32}
% Qwen2.5-0.5B & 10.74 & 11.88 & 12.09 & 13.25 & 14.41 & 10.78 &6.65 \\

\bottomrule
\end{tabular}
}
% The columns Easy(sample), Middle(sample), and Hard(sample) represent average scores according to difficulty. 
\captionsetup{font=footnotesize}
\caption{\textbf{Performance on \benchmark.} 
LLMs are scored sample-wise, subfield-wise, field-wise, and discipline-wise levels to ensure fair assessment despite imbalanced question distributions. The highest, the second-best and the third-best scores are shown in  \boxed{box}, \textbf{bold} and \underline{underlined}, respectively.}
\label{performance1}
\end{table}
}
% \newgeometry{top=3cm,bottom=3cm} % 第一页特殊边距


==> sections/results/performance_2.tex <==
\definecolor{color11}{rgb}{1, 0.8, 0.8}  % 红色20%混合
\definecolor{color12}{rgb}{1, 0.9, 0.9}  % 红色10%混合
\definecolor{color21}{RGB}{255, 224, 127}  % 更亮的黄色调，温暖
\definecolor{color22}{RGB}{255, 239, 179}  % 浅黄色调，亮度增加
\definecolor{color31}{RGB}{198, 230, 195}  % 更亮的绿色，柔和清新
\definecolor{color32}{RGB}{224, 239, 225}  % 更亮的浅绿色，清新且明亮

{
\linespread{1}
\begin{table}[H]
\footnotesize
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
% \textbf{Model} & \textbf{Agronomy} & \textbf{Economics} & \textbf{Education} & \textbf{Engineering} & \textbf{History} & \textbf{Law} & \textbf{Literature and Arts} & \textbf{Management} & \textbf{Medicine} & \textbf{Military Science} & \textbf{Philosophy} & \textbf{Science} & \textbf{Sociology}\\
\textbf{Model} & \textbf{Agr.} & \textbf{Econ.} & \textbf{Edu.} & \textbf{Eng.} & \textbf{Hist.} & \textbf{Law} & \textbf{Lit \& Arts} & \textbf{Mgt.} & \textbf{Med.} & \textbf{Mil Sci.} & \textbf{Phil.} & \textbf{Sci.} & \textbf{Soc.} \\
\midrule
\rowcolor{color11}
\multicolumn{14}{c}{\textbf{\textit{Reasoning Models}}}\\
\midrule
\rowcolor{color12}
DeepSeek-R1& \boxed{54.43}& \textbf{66.09}& \textbf{54.75}& \boxed{63.10}& \underline{55.19}& \textbf{65.24}& \underline{52.45}& \underline{57.09}& \underline{59.93}& \underline{57.07}& \textbf{63.11}& \boxed{63.69}& \boxed{67.13} \\
\rowcolor{color12}
DeepSeek-R1-Zero& \textbf{53.81}& \boxed{66.44}& \boxed{60.54}& \textbf{60.28}& \textbf{58.61}& \boxed{66.77}& \boxed{56.86}& \boxed{59.68}& \textbf{60.65}& \textbf{58.54}& \boxed{63.69}& 59.93& \boxed{67.13} \\
\rowcolor{color12}
o1-2024-12-17& \underline{50.93}& \underline{61.17}& \underline{53.31}& \underline{59.17}& \boxed{60.98}& \underline{63.87}& \textbf{55.79}& \textbf{57.29}& \boxed{62.25}& \boxed{60.49}& \underline{61.38}& \textbf{61.76}& \textbf{64.34} \\
\rowcolor{color12}
o3-mini-2025-01-31-high& 41.03& 54.07& 46.28& 56.41& 36.80& 45.73& 39.44& 51.50& 51.72& 46.34& 51.01& \underline{61.72}& \underline{46.15} \\
\rowcolor{color12}
o3-mini-2025-01-31-medium& 40.62& 51.32& 41.74& 53.83& 35.01& 43.60& 37.11& 48.50& 50.34& 45.85& 48.13& 58.79& 44.06 \\
\rowcolor{color12}
o3-mini-2025-01-31-low& 37.32& 45.25& 38.43& 48.20& 32.94& 39.79& 36.22& 43.71& 48.09& 41.46& 44.09& 53.24& 45.45 \\
\rowcolor{color12}
o1-mini-2024-09-12& 34.02& 45.02& 36.16& 45.41& 26.26& 35.98& 32.22& 40.52& 44.32& 39.51& 39.48& 51.09& 41.26 \\
\rowcolor{color12}
QwQ& 38.14& 47.77& 45.25& 43.37& 29.53& 45.88& 32.82& 41.32& 43.88& 40.00& 43.52& 46.33& 43.36 \\
\midrule
\rowcolor{color21}
\multicolumn{14}{c}{\textbf{\textit{Chat Models}}}\\
\midrule
\rowcolor{color22}
Doubao-1.5-pro-32k-250115& \boxed{50.93}& \boxed{65.06}& \textbf{55.58}& \boxed{55.60}& 42.88& \textbf{58.84}& 42.30& \textbf{53.29}& \boxed{59.13}& \textbf{54.15}& \boxed{61.96}& \boxed{55.54}& 51.75 \\
\rowcolor{color22}
Doubao-1.5-pro-32k-241225& \textbf{47.42}& \textbf{60.14}& \underline{54.75}& \underline{50.76}& 37.54& 54.12& 38.31& \underline{52.69}& \underline{54.99}& \underline{53.66}& \textbf{57.06}& \textbf{51.57}& 53.15 \\
\rowcolor{color22}
claude-3-5-sonnet-20241022& \underline{47.01}& 56.59& 53.72& 47.57& \boxed{53.56}& \boxed{60.21}& \boxed{50.42}& 51.30& 49.26& \boxed{59.51}& 52.45& 45.02& \boxed{64.34} \\
\rowcolor{color22}
qwen-max-2025-01-25& 44.33& \underline{57.50}& \boxed{56.40}& \textbf{50.81}& 44.81& 54.12& 44.93& \boxed{54.69}& \textbf{56.37}& 49.27& \underline{56.20}& 47.51& \underline{54.55} \\
\rowcolor{color22}
Llama-3.1-405B-Instruct& 43.09& 49.71& 45.45& 41.89& 50.00& \underline{55.34}& 43.20& 47.70& 49.04& 52.20& 48.41& 39.80& 49.65 \\
\rowcolor{color22}
gpt-4o-2024-11-20& 42.27& 46.74& 50.00& 42.83& \textbf{52.52}& 53.81& \textbf{46.72}& 47.31& 52.52& 52.20& 52.74& 40.67& \underline{54.55} \\
\rowcolor{color22}
gpt-4o-2024-05-13& 41.44& 40.78& 44.21& 37.47& 50.74& 52.90& 45.11& 41.32& 48.82& 50.73& 45.24& 35.41& 53.85 \\
\rowcolor{color22}
DeepSeek-V3& 41.24& 49.48& 43.80& 47.21& 47.18& 51.07& 45.23& 48.50& 46.10& 48.29& 43.23& 48.30& \textbf{55.94} \\
\rowcolor{color22}
Qwen2.5-72B-Instruct& 41.24& 46.62& 44.42& 41.12& 30.71& 45.88& 34.90& 42.32& 45.74& 45.37& 43.52& 39.33& 46.15 \\
\rowcolor{color22}
MiniMax-Text-01& 39.79& 49.60& 47.52& 44.88& 45.25& 54.27& 43.02& 48.90& 47.08& 48.29& 45.53& 43.81& 53.85 \\
\rowcolor{color22}
gpt-4o-2024-08-06& 39.59& 40.78& 44.42& 38.84& \underline{50.89}& 54.12& \underline{46.30}& 45.51& 50.49& 50.73& 47.84& 38.41& 53.85 \\
\rowcolor{color22}
Mistral-Large-Instruct-2411& 38.76& 42.27& 42.15& 39.66& 44.96& 47.87& 41.11& 43.31& 43.23& 48.78& 42.07& 39.24& 50.35 \\
\rowcolor{color22}
gemini-2.0-flash& 38.56& 45.93& 42.36& 48.37& 45.25& 49.24& 43.68& 41.32& 43.77& 51.22& 45.53& \underline{50.20}& 53.85 \\
\rowcolor{color22}
Llama-3.1-70B-Instruct& 37.11& 41.12& 41.94& 33.88& 33.09& 45.88& 35.08& 46.11& 44.21& 47.80& 42.94& 30.04& 48.25 \\
\rowcolor{color22}
Llama-3.3-70B-Instruct& 36.70& 40.55& 40.29& 36.44& 41.25& 44.66& 38.54& 45.51& 43.77& 46.34& 42.94& 34.96& 42.66 \\
\rowcolor{color22}
qwen-max-2024-09-19& 36.49& 45.02& 45.66& 39.84& 35.16& 44.05& 39.08& 45.11& 43.41& 47.32& 43.23& 38.24& 38.46 \\
\rowcolor{color22}
Qwen2.5-32B-Instruct& 36.49& 43.07& 45.45& 38.93& 30.71& 41.92& 32.76& 39.52& 42.21& 44.88& 39.19& 38.24& 39.16 \\
\rowcolor{color22}
Qwen2.5-14B-Instruct& 36.08& 37.69& 39.26& 35.87& 26.41& 37.04& 31.44& 41.52& 36.91& 38.05& 38.04& 34.20& 36.36 \\
\rowcolor{color22}
Yi-Lighting& 33.81& 39.18& 35.95& 32.53& 36.05& 37.35& 36.34& 38.12& 36.95& 42.44& 37.75& 30.85& 42.66 \\
\rowcolor{color22}
phi-4& 32.78& 40.21& 39.26& 37.27& 30.27& 41.46& 31.62& 39.12& 37.79& 39.02& 40.63& 38.87& 41.26 \\
\rowcolor{color22}
gemma-2-27b-it& 31.13& 29.32& 30.99& 26.72& 24.78& 35.06& 29.42& 34.93& 31.00& 39.02& 35.45& 24.81& 34.27 \\
\rowcolor{color22}
Qwen2.5-7B-Instruct& 29.28& 34.59& 35.33& 28.38& 22.85& 32.62& 24.28& 33.33& 32.60& 32.68& 34.58& 27.54& 30.07 \\
\rowcolor{color22}
Mistral-Small-Instruct-2409& 28.87& 26.23& 26.86& 25.25& 25.96& 30.95& 27.57& 30.54& 28.53& 34.15& 29.68& 24.17& 32.87 \\
\rowcolor{color22}
Yi-1.5-34B-Chat& 28.87& 31.27& 30.99& 25.67& 23.00& 34.45& 27.15& 31.54& 29.73& 33.17& 30.26& 23.27& 28.67 \\
\rowcolor{color22}
Mixtral-8x22B-Instruct-v0.1& 28.25& 33.45& 33.68& 29.02& 30.86& 34.60& 30.55& 35.13& 30.53& 44.39& 32.85& 26.95& 36.36 \\
\rowcolor{color22}
Mixtral-8x7B-Instruct-v0.1& 27.22& 24.51& 28.31& 21.16& 25.37& 30.79& 26.85& 26.15& 26.13& 30.73& 25.94& 18.70& 30.77 \\
\rowcolor{color22}
gemma-2-9b-it& 27.01& 27.15& 32.64& 23.24& 22.26& 28.51& 27.45& 32.14& 27.44& 34.15& 29.39& 21.26& 27.97 \\
\rowcolor{color22}
Qwen2.5-3B-Instruct& 25.36& 26.35& 30.99& 22.83& 18.55& 25.61& 22.32& 30.94& 26.82& 27.32& 27.09& 21.64& 26.57 \\
\rowcolor{color22}
granite-3.1-8b-instruct& 24.74& 20.16& 23.76& 21.60& 16.32& 24.70& 20.53& 25.15& 20.58& 27.80& 21.33& 19.70& 23.08 \\
\rowcolor{color22}
Llama-3.1-8B-Instruct& 24.74& 24.40& 29.55& 19.07& 20.03& 26.68& 20.94& 34.13& 30.20& 34.63& 27.67& 16.08& 31.47 \\
\rowcolor{color22}
gemma-2-2b-it& 24.33& 21.31& 19.42& 18.30& 17.06& 21.80& 19.21& 21.56& 19.27& 26.83& 19.60& 17.53& 20.28 \\
\rowcolor{color22}
Yi-1.5-9B-Chat& 24.12& 29.90& 30.99& 23.04& 16.91& 28.20& 20.70& 31.94& 25.74& 28.29& 27.09& 21.23& 30.77 \\
\rowcolor{color22}
K2-Chat& 22.68& 23.37& 27.27& 23.10& 16.02& 30.49& 23.39& 28.74& 23.99& 28.29& 27.09& 20.32& 25.17 \\
\rowcolor{color22}
Qwen2.5-1.5B-Instruct& 22.27& 22.57& 27.27& 17.64& 16.47& 26.37& 17.84& 24.95& 22.58& 25.37& 27.67& 16.85& 19.58 \\
\rowcolor{color22}
OLMo-2-1124-13B-Instruct& 20.82& 22.68& 25.21& 18.18& 16.91& 22.10& 19.57& 21.96& 21.81& 25.85& 27.38& 16.39& 24.48 \\
\rowcolor{color22}
OLMo-2-1124-7B-Instruct& 20.82& 14.66& 20.25& 16.52& 16.32& 18.45& 18.08& 22.95& 17.82& 23.41& 21.90& 15.64& 18.18 \\
\rowcolor{color22}
Yi-1.5-6B-Chat& 20.41& 23.83& 25.62& 18.50& 13.95& 25.61& 18.79& 24.15& 21.89& 29.27& 25.36& 17.60& 23.78 \\
\rowcolor{color22}
Mistral-7B-Instruct-v0.3& 20.00& 17.75& 18.18& 17.28& 15.88& 21.19& 21.12& 23.55& 20.04& 26.83& 22.19& 16.18& 20.98 \\
\rowcolor{color22}
granite-3.1-2b-instruct& 18.14& 19.93& 19.83& 17.64& 16.77& 23.02& 19.03& 23.15& 17.46& 22.44& 19.02& 17.09& 20.98 \\
\rowcolor{color22}
MAP-Neo-7B-Instruct-v0.1& 17.94& 17.64& 21.69& 16.79& 13.50& 21.19& 16.35& 20.96& 18.91& 25.85& 21.61& 15.99& 14.69 \\
\rowcolor{color22}
Qwen2.5-0.5B-Instruct& 16.91& 16.49& 17.98& 9.77& 10.09& 13.87& 12.89& 15.97& 14.12& 13.17& 12.68& 8.55& 12.59 \\
\midrule
\rowcolor{color31}
\multicolumn{14}{c}{\textbf{\textit{Base Models}}}\\
\midrule
\rowcolor{color32}
Qwen2.5-32B& \boxed{38.76}& \textbf{40.89}& \boxed{45.87}& \textbf{32.70}& 28.49& \textbf{39.94}& 30.91& \textbf{40.72}& \textbf{38.84}& \boxed{47.80}& \boxed{43.52}& \textbf{29.45}& \boxed{39.86} \\
\rowcolor{color32}
Qwen2.5-72B& \textbf{36.29}& \boxed{44.33}& \textbf{45.25}& \boxed{33.39}& \underline{31.31}& \boxed{44.21}& \boxed{35.50}& \boxed{43.51}& \boxed{43.12}& \textbf{46.34}& \textbf{42.94}& \underline{29.38}& \textbf{38.46} \\
\rowcolor{color32}
Qwen2.5-14B& \underline{34.02}& 34.82& \underline{40.08}& 30.26& 28.49& 36.89& 28.94& \underline{40.32}& 34.37& 40.00& 37.75& 26.68& 36.36 \\
\rowcolor{color32}
Llama-3.1-405B& 29.28& 27.95& 31.20& 23.61& \boxed{34.12}& 34.30& 30.79& 34.13& 29.47& 39.51& 31.70& 21.47& 24.48 \\
\rowcolor{color32}
Llama-3.1-70B& 28.87& 29.67& 36.36& 26.19& \textbf{32.94}& 33.38& \underline{32.64}& 36.73& 30.96& \underline{40.98}& 36.89& 23.30& 34.27 \\
\rowcolor{color32}
gemma-2-27b& 28.87& 27.26& 30.79& 24.09& 22.85& 28.96& 27.51& 32.73& 27.80& 37.56& 31.70& 21.38& 30.07 \\
\rowcolor{color32}
DeepSeek-V3-Base& 28.66& 35.17& 39.05& \underline{31.87}& 30.12& \underline{37.20}& \textbf{33.65}& 37.33& \underline{34.70}& 37.07& \underline{38.62}& \boxed{30.08}& \underline{37.76} \\
\rowcolor{color32}
Qwen2.5-7B& 28.25& 31.96& 38.02& 24.89& 22.55& 30.34& 25.06& 28.54& 30.56& 31.71& 36.60& 22.04& 34.27 \\
\rowcolor{color32}
Yi-1.5-34B& 28.25& \underline{35.85}& 37.60& 27.32& 24.63& 34.45& 30.25& 36.13& 31.18& 40.49& 35.45& 23.80& \underline{37.76} \\
\rowcolor{color32}
Mixtral-8x7B-v0.1& 28.04& 24.97& 29.34& 20.67& 23.89& 30.79& 27.27& 30.74& 25.05& 37.56& 30.84& 17.87& 28.67 \\
\rowcolor{color32}
gemma-2-9b& 27.22& 26.23& 30.99& 21.79& 21.81& 26.83& 23.81& 28.94& 26.06& 32.68& 27.09& 20.01& 27.97 \\
\rowcolor{color32}
Mistral-7B-v0.3& 25.98& 20.96& 25.62& 19.02& 14.84& 24.24& 20.11& 23.55& 22.61& 30.24& 25.94& 17.47& 18.88 \\
\rowcolor{color32}
Yi-1.5-9B& 25.77& 26.12& 34.71& 23.59& 18.69& 25.15& 23.21& 30.54& 23.85& 31.22& 28.53& 20.86& 27.97 \\
\rowcolor{color32}
Mixtral-8x22B-v0.1& 23.92& 23.94& 27.27& 22.02& 20.33& 27.59& 24.64& 30.14& 22.50& 28.78& 24.50& 20.96& 28.67 \\
\rowcolor{color32}
Llama-3.1-8B& 23.30& 22.22& 25.00& 19.56& 20.92& 26.98& 21.48& 25.95& 24.54& 33.17& 26.80& 16.62& 23.78 \\
\rowcolor{color32}
K2& 22.68& 20.62& 28.93& 20.50& 17.80& 28.35& 24.40& 27.74& 22.94& 33.17& 29.11& 18.39& 25.87 \\
\rowcolor{color32}
Qwen2.5-3B& 22.47& 23.83& 28.31& 19.74& 18.40& 26.37& 21.60& 28.14& 25.41& 30.73& 29.39& 16.54& 26.57 \\
\rowcolor{color32}
Yi-1.5-6B& 22.06& 25.89& 27.07& 19.93& 14.99& 25.46& 21.36& 26.75& 21.92& 30.73& 26.80& 17.98& 23.78 \\
\rowcolor{color32}
MAP-Neo-7B& 20.21& 18.10& 23.35& 15.43& 15.28& 21.34& 18.79& 21.76& 17.10& 24.88& 22.19& 13.16& 22.38 \\
\rowcolor{color32}
OLMo-2-1124-13B& 19.59& 20.27& 26.24& 15.21& 19.73& 22.41& 20.88& 26.15& 19.96& 25.85& 26.51& 11.93& 23.08 \\
\rowcolor{color32}
Qwen2.5-1.5B& 19.18& 20.73& 28.10& 16.50& 15.43& 21.95& 17.72& 23.35& 20.87& 24.88& 25.65& 14.48& 28.67 \\
\rowcolor{color32}
granite-3.1-2b-base& 18.76& 18.33& 23.55& 16.37& 13.80& 19.21& 16.41& 18.96& 17.39& 21.46& 22.48& 14.48& 13.99 \\
\rowcolor{color32}
OLMo-2-1124-7B& 18.35& 17.30& 25.00& 14.88& 19.14& 19.36& 17.36& 20.76& 18.73& 22.44& 22.48& 11.72& 27.27 \\
\rowcolor{color32}
gemma-2-2b& 18.35& 16.15& 19.21& 12.82& 11.72& 19.21& 15.75& 18.36& 16.52& 19.02& 19.60& 11.41& 12.59 \\
\rowcolor{color32}
granite-3.1-8b-base& 15.46& 17.87& 15.08& 16.26& 11.72& 18.29& 13.84& 14.57& 14.81& 20.49& 20.17& 15.44& 22.38 \\
\rowcolor{color32}
Qwen2.5-0.5B& 15.05& 12.37& 16.32& 10.30& 11.42& 12.96& 14.92& 11.78& 12.23& 16.59& 15.56& 8.74& 13.99 \\

\bottomrule
\end{tabular}
}
\captionsetup{font=footnotesize}
\caption{\textbf{Detailed Performance Overview on \benchmark - Pivot Table 2.} 
The table presents LLMs' performance on different disciplines. The highest score in each column is indicated with a \boxed{box}; the second-best score is in \textbf{bold}, and the third-best score is \underline{underlined}.}
\label{performance2_all}
\end{table}
}



==> sections/results/performance_2_main.tex <==
\definecolor{color11}{rgb}{1, 0.8, 0.8}  % 红色20%混合
\definecolor{color12}{rgb}{1, 0.9, 0.9}  % 红色10%混合
\definecolor{color21}{RGB}{255, 224, 127}  % 更亮的黄色调，温暖
\definecolor{color22}{RGB}{255, 239, 179}  % 浅黄色调，亮度增加
\definecolor{color31}{RGB}{198, 230, 195}  % 更亮的绿色，柔和清新
\definecolor{color32}{RGB}{224, 239, 225}  % 更亮的浅绿色，清新且明亮

{
\linespread{1.1}
\begin{table}[p]
\small
\centering
\setlength{\tabcolsep}{2pt} 

\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
% \textbf{Model} & \textbf{Agronomy} & \textbf{Economics} & \textbf{Education} & \textbf{Engineering} & \textbf{History} & \textbf{Law} & \textbf{Literature and Arts} & \textbf{Management} & \textbf{Medicine} & \textbf{Military Science} & \textbf{Philosophy} & \textbf{Science} & \textbf{Sociology}\\
\textbf{Model} & \textbf{Agr.} & \textbf{Econ.} & \textbf{Edu.} & \textbf{Eng.} & \textbf{Hist.} & \textbf{Law} & \textbf{Lit \& Arts} & \textbf{Mgt.} & \textbf{Med.} & \textbf{Mil Sci.} & \textbf{Phil.} & \textbf{Sci.} & \textbf{Soc.} \\
\midrule
\rowcolor{color11}
\multicolumn{14}{c}{\textbf{\textit{Reasoning Models}}}\\
\midrule
\rowcolor{color12}
DeepSeek-R1& \boxed{54.43}& \textbf{66.09}& \textbf{54.75}& \boxed{63.10}& \underline{55.19}& \textbf{65.24}& \underline{52.45}& \underline{57.09}& \underline{59.93}& \underline{57.07}& \textbf{63.11}& \boxed{63.69}& \boxed{67.13} \\
\rowcolor{color12}
DeepSeek-R1-Zero& \textbf{53.81}& \boxed{66.44}& \boxed{60.54}& \textbf{60.28}& \textbf{58.61}& \boxed{66.77}& \boxed{56.86}& \boxed{59.68}& \textbf{60.65}& \textbf{58.54}& \boxed{63.69}& 59.93& \boxed{67.13} \\
\rowcolor{color12}
o1-2024-12-17& \underline{50.93}& \underline{61.17}& \underline{53.31}& \underline{59.17}& \boxed{60.98}& \underline{63.87}& \textbf{55.79}& \textbf{57.29}& \boxed{62.25}& \boxed{60.49}& \underline{61.38}& \textbf{61.76}& \textbf{64.34} \\
\rowcolor{color12}
o3-mini-2025-01-31-high& 41.03& 54.07& 46.28& 56.41& 36.80& 45.73& 39.44& 51.50& 51.72& 46.34& 51.01& \underline{61.72}& \underline{46.15} \\
\rowcolor{color12}
o3-mini-2025-01-31-medium& 40.62& 51.32& 41.74& 53.83& 35.01& 43.60& 37.11& 48.50& 50.34& 45.85& 48.13& 58.79& 44.06 \\
\rowcolor{color12}
o3-mini-2025-01-31-low& 37.32& 45.25& 38.43& 48.20& 32.94& 39.79& 36.22& 43.71& 48.09& 41.46& 44.09& 53.24& 45.45 \\
\rowcolor{color12}
o1-mini-2024-09-12& 34.02& 45.02& 36.16& 45.41& 26.26& 35.98& 32.22& 40.52& 44.32& 39.51& 39.48& 51.09& 41.26 \\
\rowcolor{color12}
QwQ& 38.14& 47.77& 45.25& 43.37& 29.53& 45.88& 32.82& 41.32& 43.88& 40.00& 43.52& 46.33& 43.36 \\
\midrule
\rowcolor{color21}
\multicolumn{14}{c}{\textbf{\textit{Chat Models}}}\\
\midrule
\rowcolor{color22}
Doubao-1.5-pro-32k-250115& \boxed{50.93}& \boxed{65.06}& \textbf{55.58}& \boxed{55.60}& 42.88& \textbf{58.84}& 42.30& \textbf{53.29}& \boxed{59.13}& \textbf{54.15}& \boxed{61.96}& \boxed{55.54}& 51.75 \\
\rowcolor{color22}
Doubao-1.5-pro-32k-241225& \textbf{47.42}& \textbf{60.14}& \underline{54.75}& \underline{50.76}& 37.54& 54.12& 38.31& \underline{52.69}& \underline{54.99}& \underline{53.66}& \textbf{57.06}& \textbf{51.57}& 53.15 \\
\rowcolor{color22}
claude-3-5-sonnet-20241022& \underline{47.01}& 56.59& 53.72& 47.57& \boxed{53.56}& \boxed{60.21}& \boxed{50.42}& 51.30& 49.26& \boxed{59.51}& 52.45& 45.02& \boxed{64.34} \\
\rowcolor{color22}
qwen-max-2025-01-25& 44.33& \underline{57.50}& \boxed{56.40}& \textbf{50.81}& 44.81& 54.12& 44.93& \boxed{54.69}& \textbf{56.37}& 49.27& \underline{56.20}& 47.51& \underline{54.55} \\
\rowcolor{color22}
Llama-3.1-405B-Instruct& 43.09& 49.71& 45.45& 41.89& 50.00& \underline{55.34}& 43.20& 47.70& 49.04& 52.20& 48.41& 39.80& 49.65 \\
\rowcolor{color22}
gpt-4o-2024-11-20& 42.27& 46.74& 50.00& 42.83& \textbf{52.52}& 53.81& \textbf{46.72}& 47.31& 52.52& 52.20& 52.74& 40.67& \underline{54.55} \\
\rowcolor{color22}
gpt-4o-2024-05-13& 41.44& 40.78& 44.21& 37.47& 50.74& 52.90& 45.11& 41.32& 48.82& 50.73& 45.24& 35.41& 53.85 \\
\rowcolor{color22}
DeepSeek-V3& 41.24& 49.48& 43.80& 47.21& 47.18& 51.07& 45.23& 48.50& 46.10& 48.29& 43.23& 48.30& \textbf{55.94} \\
\rowcolor{color22}
Qwen2.5-72B-Instruct& 41.24& 46.62& 44.42& 41.12& 30.71& 45.88& 34.90& 42.32& 45.74& 45.37& 43.52& 39.33& 46.15 \\
\rowcolor{color22}
MiniMax-Text-01& 39.79& 49.60& 47.52& 44.88& 45.25& 54.27& 43.02& 48.90& 47.08& 48.29& 45.53& 43.81& 53.85 \\
\rowcolor{color22}
gpt-4o-2024-08-06& 39.59& 40.78& 44.42& 38.84& \underline{50.89}& 54.12& \underline{46.30}& 45.51& 50.49& 50.73& 47.84& 38.41& 53.85 \\
\rowcolor{color22}
Mistral-Large-Instruct-2411& 38.76& 42.27& 42.15& 39.66& 44.96& 47.87& 41.11& 43.31& 43.23& 48.78& 42.07& 39.24& 50.35 \\
\rowcolor{color22}
gemini-2.0-flash& 38.56& 45.93& 42.36& 48.37& 45.25& 49.24& 43.68& 41.32& 43.77& 51.22& 45.53& \underline{50.20}& 53.85 \\
\rowcolor{color22}
Llama-3.1-70B-Instruct& 37.11& 41.12& 41.94& 33.88& 33.09& 45.88& 35.08& 46.11& 44.21& 47.80& 42.94& 30.04& 48.25 \\
\rowcolor{color22}
Llama-3.3-70B-Instruct& 36.70& 40.55& 40.29& 36.44& 41.25& 44.66& 38.54& 45.51& 43.77& 46.34& 42.94& 34.96& 42.66 \\
\rowcolor{color22}
qwen-max-2024-09-19& 36.49& 45.02& 45.66& 39.84& 35.16& 44.05& 39.08& 45.11& 43.41& 47.32& 43.23& 38.24& 38.46 \\
\rowcolor{color22}
Qwen2.5-32B-Instruct& 36.49& 43.07& 45.45& 38.93& 30.71& 41.92& 32.76& 39.52& 42.21& 44.88& 39.19& 38.24& 39.16 \\
\rowcolor{color22}
Qwen2.5-14B-Instruct& 36.08& 37.69& 39.26& 35.87& 26.41& 37.04& 31.44& 41.52& 36.91& 38.05& 38.04& 34.20& 36.36 \\
\rowcolor{color22}
Yi-Lighting& 33.81& 39.18& 35.95& 32.53& 36.05& 37.35& 36.34& 38.12& 36.95& 42.44& 37.75& 30.85& 42.66 \\
\rowcolor{color22}
Phi-4& 32.78& 40.21& 39.26& 37.27& 30.27& 41.46& 31.62& 39.12& 37.79& 39.02& 40.63& 38.87& 41.26 \\
\rowcolor{color22}
Gemma-2-27B-it& 31.13& 29.32& 30.99& 26.72& 24.78& 35.06& 29.42& 34.93& 31.00& 39.02& 35.45& 24.81& 34.27 \\
\rowcolor{color22}
Qwen2.5-7B-Instruct& 29.28& 34.59& 35.33& 28.38& 22.85& 32.62& 24.28& 33.33& 32.60& 32.68& 34.58& 27.54& 30.07 \\
% \rowcolor{color22}
% Mistral-Small-Instruct-2409& 28.87& 26.23& 26.86& 25.25& 25.96& 30.95& 27.57& 30.54& 28.53& 34.15& 29.68& 24.17& 32.87 \\
% \rowcolor{color22}
% Yi-1.5-34B-Chat& 28.87& 31.27& 30.99& 25.67& 23.00& 34.45& 27.15& 31.54& 29.73& 33.17& 30.26& 23.27& 28.67 \\
\rowcolor{color22}
Mixtral-8x22B-Instruct-v0.1& 28.25& 33.45& 33.68& 29.02& 30.86& 34.60& 30.55& 35.13& 30.53& 44.39& 32.85& 26.95& 36.36 \\
% \rowcolor{color22}
% Mixtral-8x7B-Instruct-v0.1& 27.22& 24.51& 28.31& 21.16& 25.37& 30.79& 26.85& 26.15& 26.13& 30.73& 25.94& 18.70& 30.77 \\
% \rowcolor{color22}
% Gemma-2-9B-it& 27.01& 27.15& 32.64& 23.24& 22.26& 28.51& 27.45& 32.14& 27.44& 34.15& 29.39& 21.26& 27.97 \\
\rowcolor{color22}
Qwen2.5-3B-Instruct& 25.36& 26.35& 30.99& 22.83& 18.55& 25.61& 22.32& 30.94& 26.82& 27.32& 27.09& 21.64& 26.57 \\
\rowcolor{color22}
Granite-3.1-8B-instruct& 24.74& 20.16& 23.76& 21.60& 16.32& 24.70& 20.53& 25.15& 20.58& 27.80& 21.33& 19.70& 23.08 \\
% \rowcolor{color22}
% Llama-3.1-8B-Instruct& 24.74& 24.40& 29.55& 19.07& 20.03& 26.68& 20.94& 34.13& 30.20& 34.63& 27.67& 16.08& 31.47 \\
% \rowcolor{color22}
% gemma-2-2b-it& 24.33& 21.31& 19.42& 18.30& 17.06& 21.80& 19.21& 21.56& 19.27& 26.83& 19.60& 17.53& 20.28 \\
% \rowcolor{color22}
% Yi-1.5-9B-Chat& 24.12& 29.90& 30.99& 23.04& 16.91& 28.20& 20.70& 31.94& 25.74& 28.29& 27.09& 21.23& 30.77 \\
% \rowcolor{color22}
% K2-Chat& 22.68& 23.37& 27.27& 23.10& 16.02& 30.49& 23.39& 28.74& 23.99& 28.29& 27.09& 20.32& 25.17 \\
\rowcolor{color22}
Qwen2.5-1.5B-Instruct& 22.27& 22.57& 27.27& 17.64& 16.47& 26.37& 17.84& 24.95& 22.58& 25.37& 27.67& 16.85& 19.58 \\
\rowcolor{color22}
OLMo-2-1124-13B-Instruct& 20.82& 22.68& 25.21& 18.18& 16.91& 22.10& 19.57& 21.96& 21.81& 25.85& 27.38& 16.39& 24.48 \\
% \rowcolor{color22}
% OLMo-2-1124-7B-Instruct& 20.82& 14.66& 20.25& 16.52& 16.32& 18.45& 18.08& 22.95& 17.82& 23.41& 21.90& 15.64& 18.18 \\
\rowcolor{color22}
Yi-1.5-6B-Chat& 20.41& 23.83& 25.62& 18.50& 13.95& 25.61& 18.79& 24.15& 21.89& 29.27& 25.36& 17.60& 23.78 \\
% \rowcolor{color22}
% Mistral-7B-Instruct-v0.3& 20.00& 17.75& 18.18& 17.28& 15.88& 21.19& 21.12& 23.55& 20.04& 26.83& 22.19& 16.18& 20.98 \\
% \rowcolor{color22}
% granite-3.1-2b-instruct& 18.14& 19.93& 19.83& 17.64& 16.77& 23.02& 19.03& 23.15& 17.46& 22.44& 19.02& 17.09& 20.98 \\
\rowcolor{color22}
MAP-Neo-7B-Instruct-v0.1& 17.94& 17.64& 21.69& 16.79& 13.50& 21.19& 16.35& 20.96& 18.91& 25.85& 21.61& 15.99& 14.69 \\
\rowcolor{color22}
Qwen2.5-0.5B-Instruct& 16.91& 16.49& 17.98& 9.77& 10.09& 13.87& 12.89& 15.97& 14.12& 13.17& 12.68& 8.55& 12.59 \\
\midrule
\rowcolor{color31}
\multicolumn{14}{c}{\textbf{\textit{Base Models}}}\\
\midrule
\rowcolor{color32}
Qwen2.5-32B& \boxed{38.76}& \textbf{40.89}& \boxed{45.87}& \textbf{32.70}& 28.49& \textbf{39.94}& 30.91& \textbf{40.72}& \textbf{38.84}& \boxed{47.80}& \boxed{43.52}& \textbf{29.45}& \boxed{39.86} \\
\rowcolor{color32}
Qwen2.5-72B& \textbf{36.29}& \boxed{44.33}& \textbf{45.25}& \boxed{33.39}& \underline{31.31}& \boxed{44.21}& \boxed{35.50}& \boxed{43.51}& \boxed{43.12}& \textbf{46.34}& \textbf{42.94}& \underline{29.38}& \textbf{38.46} \\
\rowcolor{color32}
Qwen2.5-14B& \underline{34.02}& 34.82& \underline{40.08}& 30.26& 28.49& 36.89& 28.94& \underline{40.32}& 34.37& 40.00& 37.75& 26.68& 36.36 \\
\rowcolor{color32}
Llama-3.1-405B& 29.28& 27.95& 31.20& 23.61& \boxed{34.12}& 34.30& 30.79& 34.13& 29.47& 39.51& 31.70& 21.47& 24.48 \\
\rowcolor{color32}
Llama-3.1-70B& 28.87& 29.67& 36.36& 26.19& \textbf{32.94}& 33.38& \underline{32.64}& 36.73& 30.96& \underline{40.98}& 36.89& 23.30& 34.27 \\
\rowcolor{color32}
Gemma-2-27B& 28.87& 27.26& 30.79& 24.09& 22.85& 28.96& 27.51& 32.73& 27.80& 37.56& 31.70& 21.38& 30.07 \\
\rowcolor{color32}
DeepSeek-V3-Base& 28.66& 35.17& 39.05& \underline{31.87}& 30.12& \underline{37.20}& \textbf{33.65}& 37.33& \underline{34.70}& 37.07& \underline{38.62}& \boxed{30.08}& \underline{37.76} \\
\rowcolor{color32}
Qwen2.5-7B& 28.25& 31.96& 38.02& 24.89& 22.55& 30.34& 25.06& 28.54& 30.56& 31.71& 36.60& 22.04& 34.27 \\
\rowcolor{color32}
Yi-1.5-34B& 28.25& \underline{35.85}& 37.60& 27.32& 24.63& 34.45& 30.25& 36.13& 31.18& 40.49& 35.45& 23.80& \underline{37.76} \\
\rowcolor{color32}
Mixtral-8x7B-v0.1& 28.04& 24.97& 29.34& 20.67& 23.89& 30.79& 27.27& 30.74& 25.05& 37.56& 30.84& 17.87& 28.67 \\
\rowcolor{color32}
Gemma-2-9B& 27.22& 26.23& 30.99& 21.79& 21.81& 26.83& 23.81& 28.94& 26.06& 32.68& 27.09& 20.01& 27.97 \\
\rowcolor{color32}
Mistral-7B-v0.3& 25.98& 20.96& 25.62& 19.02& 14.84& 24.24& 20.11& 23.55& 22.61& 30.24& 25.94& 17.47& 18.88 \\
% \rowcolor{color32}
% Yi-1.5-9B& 25.77& 26.12& 34.71& 23.59& 18.69& 25.15& 23.21& 30.54& 23.85& 31.22& 28.53& 20.86& 27.97 \\
\rowcolor{color32}
Mixtral-8x22B-v0.1& 23.92& 23.94& 27.27& 22.02& 20.33& 27.59& 24.64& 30.14& 22.50& 28.78& 24.50& 20.96& 28.67 \\
% \rowcolor{color32}
% Llama-3.1-8B& 23.30& 22.22& 25.00& 19.56& 20.92& 26.98& 21.48& 25.95& 24.54& 33.17& 26.80& 16.62& 23.78 \\
% \rowcolor{color32}
% K2& 22.68& 20.62& 28.93& 20.50& 17.80& 28.35& 24.40& 27.74& 22.94& 33.17& 29.11& 18.39& 25.87 \\
\rowcolor{color32}
Qwen2.5-3B& 22.47& 23.83& 28.31& 19.74& 18.40& 26.37& 21.60& 28.14& 25.41& 30.73& 29.39& 16.54& 26.57 \\
% \rowcolor{color32}
% Yi-1.5-6B& 22.06& 25.89& 27.07& 19.93& 14.99& 25.46& 21.36& 26.75& 21.92& 30.73& 26.80& 17.98& 23.78 \\
\rowcolor{color32}
MAP-Neo-7B& 20.21& 18.10& 23.35& 15.43& 15.28& 21.34& 18.79& 21.76& 17.10& 24.88& 22.19& 13.16& 22.38 \\
\rowcolor{color32}
OLMo-2-1124-13B& 19.59& 20.27& 26.24& 15.21& 19.73& 22.41& 20.88& 26.15& 19.96& 25.85& 26.51& 11.93& 23.08 \\
\rowcolor{color32}
Qwen2.5-1.5B& 19.18& 20.73& 28.10& 16.50& 15.43& 21.95& 17.72& 23.35& 20.87& 24.88& 25.65& 14.48& 28.67 \\
% \rowcolor{color32}
% granite-3.1-2b-base& 18.76& 18.33& 23.55& 16.37& 13.80& 19.21& 16.41& 18.96& 17.39& 21.46& 22.48& 14.48& 13.99 \\
% \rowcolor{color32}
% OLMo-2-1124-7B& 18.35& 17.30& 25.00& 14.88& 19.14& 19.36& 17.36& 20.76& 18.73& 22.44& 22.48& 11.72& 27.27 \\
% \rowcolor{color32}
% gemma-2-2b& 18.35& 16.15& 19.21& 12.82& 11.72& 19.21& 15.75& 18.36& 16.52& 19.02& 19.60& 11.41& 12.59 \\
\rowcolor{color32}
Granite-3.1-8B-Base& 15.46& 17.87& 15.08& 16.26& 11.72& 18.29& 13.84& 14.57& 14.81& 20.49& 20.17& 15.44& 22.38 \\
\rowcolor{color32}
Qwen2.5-0.5B& 15.05& 12.37& 16.32& 10.30& 11.42& 12.96& 14.92& 11.78& 12.23& 16.59& 15.56& 8.74& 13.99 \\

\bottomrule
\end{tabular}
}
\captionsetup{font=footnotesize}
\caption{\textbf{Performance on \benchmark.} 
We present LLMs' performance on different disciplines. The highest, the second-best and the third-best scores are shown in  \boxed{box}, \textbf{bold} and \underline{underlined}, respectively.}
\label{performance2}
\end{table}
}


